Query Understanding in the Age of Large Language Models

Querying, conversing, and controlling search and information-seeking interfaces using natural language are fast becoming ubiquitous with the rise and adoption of large-language models (LLM). In this position paper, we describe a generic framework for interactive query-rewriting using LLMs. Our proposal aims to unfold new opportunities for improved and transparent intent understanding while building high-performance retrieval systems using LLMs. A key aspect of our framework is the ability of the rewriter to fully specify the machine intent by the search engine in natural language that can be further refined, controlled, and edited before the final retrieval phase. The ability to present, interact, and reason over the underlying machine intent in natural language has profound implications on transparency, ranking performance, and a departure from the traditional way in which supervised signals were collected for understanding intents. We detail the concept, backed by initial experiments, along with open questions for this interactive query understanding framework.

==> SIGIR2023/tables/table-anecdotal.tex <==

\begin{table*}
    \centering
    \scriptsize
    \begin{tabularx}{\textwidth}{crl}
        \toprule
        \multicolumn{2}{r}{\textbf{Queries}} & \textbf{Intents} \\
        \midrule
        \multicolumn{3}{l}{\textbf{Query}: \texttt{Commodore}}\\
        \cmidrule{1-2}
        \parbox[b]{0pt}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Intents}}}
        & \bf 1 & A commodore's ship is typically designated by the flying of a Broad pennant, as opposed to an admiral's flag. \\
        & \bf 2 & \green{Commodore is a naval rank used in many navies that is superior to a navy captain, but below a rear admiral.} \\
        & \bf 3 & It is sometimes abbreviated: as "Cdre" in British Royal Navy, "CDRE" in the US Navy [...] \\
        & \bf 4 & Commodore (rank). \\
        & \bf 5 & Non-English-speaking nations often use the rank of flotilla admiral or counter admiral [...] \\
        \midrule
                \bottomrule
    \end{tabularx}
    \caption{Example EXAMPLE TABLE TO CONTAIN examples...\green{highlighted}.}
    \label{tab:fever_examples}
\end{table*}


==> SIGIR2023/tables/table-ranker.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\newcommand{\mycomment}[1]{}

\mycomment {
\begin{table}[]
\caption{Results for zero-shot retrieval using rewritten queries on BEIR Scifact}
\begin{tabular}{l|l|l}
\textbf{Method}                     & \textbf{NDCG@10}    & \textbf{R@100} \\ \hline
BM25                                & 0.665               & 0.921          \\\hline
tas-b                               & 0.643               & 0.891          \\\hline
RM3+BM25                            & \textbf{0.672}      & 0.918          \\\hline
KL+BM25                             & 0.652               & \textbf{0.922} \\\hline
QE+BM25                             & 0.672               & 0.918          \\\hline
BART(topic-intent) + BM25           & 0.592               & 0.892          \\\hline
BART(topic+paa-target) +BM25        & 0.273               & 0.573          \\\hline
Gpt3 (in context) + bm25            & 0.646 (beats tas-b) & 0.878          \\\hline
Gpt3 (in context) + bm25 (keywords) &                     &                \\\hline
Gpt3 (in context) + tas-b           & 0.602               & 0.858          \\\hline
BART(topic+paa-target) +tas-b       & 0.496               & 0.800          \\\hline
BART(topic-intent) + tas-b          & 0.569               & 0.873          \\\hline
Gpt3 prompt1 + bm25                 & 0.602               & 0.883          \\\hline
Gpt3 prompt1 + tas-b                & 0.570               & 0.862          \\\hline
Gpt3 prompt2 + bm25                 & 0.628               & 0.865          \\\hline
Gpt3 prompt2 + tas-b                & 0.590               & 0.827         \\\hline
\end{tabular}
\end{table}

\\
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Results for zero-shot retrieval using rewritten queries on BEIR Nfcorpus}
\begin{tabular}{lll}
                                    &                  &                                           \\\hline
\textbf{Method}                     & \textbf{NDCG@10} & \textbf{R@100}                            \\\hline
BM25                                & 0.323            & 0.244                                     \\\hline
tas-b                               & 0.319            & 0.280                                     \\\hline
RM3+BM25                            & \textbf{0.328}   & 0.296                                     \\\hline
KL+BM25                             & 0.325            & \textbf{0.296}                            \\\hline
QE+BM25                             & 0.322            & 0.244                                     \\\hline
BART(topic-intent) + BM25           & 0.225            & 0.227                                     \\\hline
BART(topic+paa-target) +BM25        & 0.197            & 0.208                                     \\\hline
Gpt3 (in context) + bm25            & 0.262            & 0.254                                     \\\hline
Gpt3 (in context) + bm25 (keywords) & 0.298            & 0.264                                     \\\hline
Gpt3 (in context) + tas-b           & 0.298            & \textbf{0.284 (better than default)}      \\\hline
BART(topic+paa-target) +tas-b       & 0.220            & 0.228                                     \\\hline
BART(topic-intent) + tas-b          & 0.253            & 0.242                                     \\\hline
Gpt3 prompt1 + bm25                 & 0.283            & 0.274                                     \\\hline
Gpt3 prompt1 + tas-b                & 0.296            & \textbf{0.287(better than default tas-b)} \\\hline
Gpt3 prompt2 + bm25                 & 0.292            & 0.244                                     \\\hline
Gpt3 prompt2 + bm25 (keywords)      & 0.304            & 0.248                                     \\\hline
Gpt3 prompt2 +  tas-b               & 0.300            & 0.274                                      \\\hline
\end{tabular}
\end{table*}
}

==> SIGIR2023/tables/table-reranking.tex <==
\begin{table}
    \centering
    \begin{tabular}{llll}
        \toprule
            \textit{\textbf{Models}}
            & $\textbf{MAP}$ & $\textbf{RR}$ & $\textbf{nDCG@10}$\\
        \midrule
\bert{} Baseline & 0.218 & 0.783 & 0.492 \\
\bart{} (topic-target)&	0.222\up{1.7} &	0.759\up{3.1} &	0.487\down{1.1}\\
\bart{} (topic+paa-target) &	\textbf{0.226\up{3.8}} &	0.824\up{5.2} &	0.497\up{0.89} \\
\textbf{\gptt{} (in context)} & 0.223\up{2.2} & \textbf{0.824\up{5.3}} & \textbf{0.513\up{4.5}} \\
\gptt{} (prompt1) & 0.219\up{0.32} & 0.801\up{2.3} & 0.486\down{1.22}\\
\gptt{} (prompt2) & 0.220\up{0.78} & 0.774\down{1.2} & 0.473\down{4.0}\\

        \bottomrule        
    \end{tabular}
    % }
    
    \caption{Ranking performance of \bert{} model trained using query expansions from different query generative models on \trecdl{} '19. We show the relative improvement of our approaches against a baseline(without query expansion)  in parentheses.}
    \vspace{-5mm}
    \label{tab:reranking-expanded-queries-msmarco}
\end{table}


==> SIGIR2023/tables/table-rewriter.tex <==
\begin{table}[]
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Method}           & \textbf{P}     & \textbf{R}     & \textbf{F1}    & \textbf{RougeL} \\
\hline

GPT2                      & 0.457          & 0.447          & 0.451          & 7.47            \\
Bart (topic-target)       & 0.792          & 0.791          & 0.792          & 28.89           \\
Bart (topic+paa - target) & 0.777          & 0.783          & 0.779          & 25.85           \\
\gptt{} (in context)         & \textbf{0.817} & \textbf{0.818} & \textbf{0.817} & \textbf{34.68}  \\
\gptt{} (prompt1)            & 0.727          & 0.743          & 0.734          & 14.38          \\
\gptt{} (prompt2)            & 0.811          & 0.792          & 0.801          & 32.07           \\

\hline
\end{tabular}
\caption{BERTScore and ROUGEL scores for different rewrites on TREC web 2012}
\label{tab:rewriter}
\end{table}
